Abstraqt: Analysis of Quantum Circuits via Abstract Stabilizer Simulation

Stabilizer simulation can efficiently simulate an important class of quantum circuits consisting exclusively of Clifford gates. However, all existing extensions of this simulation to arbitrary quantum circuits including non-Clifford gates suffer from an exponential runtime. To address this challenge, we present a novel approach for efficient stabilizer simulation on arbitrary quantum circuits, at the cost of lost precision. Our key idea is to compress an exponential sum representation of the quantum state into a single abstract summand covering (at least) all occurring summands. This allows us to introduce an abstract stabilizer simulator that efficiently manipulates abstract summands by over-approximating the effect of circuit operations including Clifford gates, non-Clifford gates, and (internal) measurements. We implemented our abstract simulator in a tool called Abstraqt and experimentally demonstrate that Abstraqt can establish circuit properties intractable for existing techniques.

==> figures/inkscape-header.tex <==
% Description: Convenience header for usage with inkscape
%
% Usage:
% - Open inkscape
% - Extensions -> TexText
% - Select this header as "Preamble File"
%
% Configure:
% - Comment out the appropriate packages (depending on your template)

%%%%%%%
% ACM %
%%%%%%%
% Conferences with this template
% - PLDI: Conference on Programming Language Design and Implementation
% - POPL: Principles of Programming Languages
% - CCS: Conference on Computer and Communications Security

% \usepackage[tt=false, type1=true]{libertine}
% \usepackage[libertine]{newtxmath}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%
% ACM with beramono %
%%%%%%%%%%%%%%%%%%%%%
% has a nice monospace font

\usepackage[tt=false, type1=true]{libertine}
\usepackage[libertine]{newtxmath}
\usepackage[scaled=0.8]{beramono} % necessary for nice font in code
\usepackage[T1]{fontenc}

\usepackage{tikz}
\usetikzlibrary{matrix}
\usetikzlibrary{calc, backgrounds}
\usetikzlibrary{fadings}

\tikzstyle{split} = [
	rounded corners=5,
	fill=\backgroundcolor,
	draw=\backgroundcolor,
	line width=#1
]
\tikzset{split/.default=-0.5cm}

\usepackage{qcircuit}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{braket}
\usepackage{ifthen}
\usepackage{xifthen}

% identity
\newcommand{\I}[1][]{\ensuremath{\mathbb{I}_{#1}}}
\newcommand{\abe}[1]{\boldsymbol{#1}} % abstract element

\newcommand{\applyat}[2][]{{#2_{\ifthenelse{\isempty{#1}}{}{(#1)}}}}

% pauli matrices
\newcommand{\pauliformat}[2]{\ensuremath{\applyat[#2]{\mathit{#1}}}}
\newcommand{\X}[1][]{\pauliformat{X}{#1}}
\newcommand{\Y}[1][]{\pauliformat{Y}{#1}}
\newcommand{\Z}[1][]{\pauliformat{Z}{#1}}
\newcommand{\T}[1][]{\pauliformat{T}{#1}}
\newcommand{\pref}[1]{\textswab{f}\left(#1\right)} % prefactor
\newcommand{\bare}[1]{\textswab{b}(#1)}
\newcommand{\grppref}[2]{\textswab{F}\left(#1, #2\right)}
\renewcommand{\i}[0]{{\rm i}}
\newcommand{\ie}[0]{i.e., }


%needed
\newcommand{\matrixspace}{2}
\newcommand{\tfact}{\ensuremath{e^{\i\pi/4}}}
\newcommand{\inset}[1]{\{{#1}\}} % abstract element
\newcommand{\scalmult}{ }
\newcommand{\scaleeq}{0.5}

%%%%%%%%%%%%%%%%%
% IEEE standard %
%%%%%%%%%%%%%%%%%
% Conferences with this template:
% - S&P: Symposium on Security and Privacy

% \usepackage{mathptmx}
% \usepackage[T1]{fontenc}

%%%%%%%%%%%%%%%%%%%%%%
% IEEE no times math %
%%%%%%%%%%%%%%%%%%%%%%
% has nicer math

% \usepackage{times}
% \usepackage[T1]{fontenc}


==> headers/lqa/abbreviations.tex <==
% Description: This file defines commands for common abbreviations
%
% Usage: \input{headers/lqa/abbreviations}

% The Backslash between `.` and ` ` is needed to ensure the white-space is an
% inter-word space, not a inter-sentence space.
%
% Details:
% - https://tex.stackexchange.com/questions/2229/is-a-period-after-an-abbreviation-the-same-as-an-end-of-sentence-period
% - https://stackoverflow.com/questions/2024338/latex-sometimes-puts-too-much-or-too-little-space-after-periods/2024341

\newcommand{\eg}{e.g., }
\newcommand{\ie}{i.e., }
\newcommand{\etc}{etc.}
\newcommand{\cp}{{cp.\ }}
\newcommand{\nth}[1]{$#1^\text{th}$}
\newcommand{\wrt}{{w.r.t.\ }}
